Real-Time Generation of Near-Minimum-Energy Trajectories via Constraint-Informed Residual Learning

Industrial robotics demands significant energy to operate, making energy-reduction methodologies increasingly important. Strategies for planning minimum-energy trajectories typically involve solving nonlinear optimal control problems (OCPs), which rarely cope with real-time requirements. In this paper, we propose a paradigm for generating near minimum-energy trajectories for manipulators by learning from optimal solutions. Our paradigm leverages a residual learning approach, which embeds boundary conditions while focusing on learning only the adjustments needed to steer a standard solution to an optimal one. Compared to a computationally expensive OCP-based planner, our paradigm achieves 87.3% of the performance near the training dataset and 50.8% far from the dataset, while being two to three orders of magnitude faster.

==> introduction.tex <==
\section{INTRODUCTION}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.98\linewidth]{abstract_v3.eps}
  \caption{ Schematic of the proposed \textit{residual} learning paradigm. }
  \label{fig:abstract}
\end{figure}


   
% \subsection{Motivation}
% -------------- The setting -------------- %
The emergence of ``green'' policies in industry is crucial for mitigating climate change. In the context of robotics, enhancing the efficiency of robotic systems can significantly reduce energy consumption and operational costs \cite{carabin2017review}.

% ---------------- Zoom in ---------------- %
Trajectory Optimization (TO) has emerged as a cost-effective approach for cutting energy consumption of robotic systems, such as single-axis systems \cite{lenzo2024real}, quadrotors \cite{morbidi2021practical}, and manipulators \cite{field1996iterative}.
In these examples, TO solves the problem of finding a trajectory that minimizes energy expenditure, which requires solving the associated Optimal Control Problem (OCP), which rarely has closed-form solutions. 
% Closed-form solutions for OCPs are rarely available, necessitating the use of numerical methods. 
Two major families of numerical methods can be distinguished: (i) direct and (ii) indirect methods \cite{bryson2018applied}. 
The former transform the $\infty$-dimensional optimization problem into a non-linear programming problem (NLP). Alternatively, the seconds formulate the problem as a Two-Point Boundary Value Problem (TPBVP) resulting from the Pontryagin Maximum Principle (PMP).
% Direct methods discretize the problem, transforming the $\infty$-dimensional optimization problem into a finite one, generally resulting in a NonLinear Programming problem (NLP). Alternatively, indirect methods attempt to solve the Two-Point Boundary Value Problem (TPBVP) resulting from the Pontryagin Maximum Principle (PMP), but these methods usually struggle to incorporate state constraints \cite{Diehl2018}.

However, the computational cost arising from the NLP or TPBVP \textit{numerical routines} makes Real-Time (RT) generation challenging, except for simple systems \cite{wang2013hamiltonian,lenzo2024real}.
RT trajectory generation is necessary for flexible automation, where precomputed (offline) trajectories are impractical.
% However, flexible automation requires robots to adapt to new scenarios by re-planning their trajectories. This makes it impractical to rely on precomputed (offline) trajectories since new ones must be generated during operation. 
Given these challenges, this letter aims to develop an RT capable method for generating near-minimum-energy OCPs solutions. \\
% RT capable solutions to the minimum-energy OCP are therefore necessary and represent the intended goal of this letter.
% ======================================
% ------------- The story so far ------------- %
% \subsection{Related works}
% As discussed, the slow solution of OCP relies on 
% generation of optimal solutions is due to the necessity of
 % solving computationally demanding numerical routines. Avoiding these routines, for instance by using \textbf{explicit} solutions of the OCP can therefore speed up the generation process.
A main idea to speed up the generation process is to avoid the \textit{numerical routines} and to use \textbf{explicit} solutions.
An early example can be seen in \cite{bemporad2000explicit}, where precomputed solutions were deployed online for a Model Predictive Control (MPC) application. %, leveraging the known structure of the solution.
% ----------------- dynamic movement primitives ----------------- %
% Another approach is based on Dynamic Movement Primitives (DMPs). DMPs rely on learning a stable, potentially nonlinear dynamic attractor system that is influenced by external forces to produce a desired motion \cite{ijspeert2002movement}. Examples include applications for quadcopters \cite{tomic2014learning} and manipulators \cite{haddadin2016optimal}.
However, a clear structure for the solution is not always available. Recently, data-driven methods have emerged as a viable option for speeding up the TO problem \cite{hauser2016learning, sambharya2023end, cheng2018real, zang2022machine, tang2019data, sanchez2018real, zhu2019deep, tailor2019learning, ferede2024end, tang2018learning, banerjee2020learning, wu2024deep, berniker2015deep, Bency2019, hochreiter1997long, vaswani2017attention, guffanti2024transformers, celestini2024transformer, briden2023constraint}. Regressors can be trained using optimal trajectories to learn mappings from the inputs of a problem to convenient outputs.
% Representative robotic problems were studied in \cite{hauser2016learning}, where input-solution mappings were learned using a k-Nearest Neighbor (k-NN) algorithm. In \cite{sambharya2023end}, Neural Networks (NN) were used to accelerate the solution of Quadratic Programming (QP) problems. Focusing in robotic TO problems,
Four main categories of methods can be distinguished based on their strategies: (i) indirect methods, (ii) state feedback methods, (iii) parameterized solution methods, and, (iv) recurrent neural network-based methods.
% ------------------ indirect methods ------------------ %
Indirect methods leverage the PMP ordinary differential equations to retrieve the solution. The regressor is used to learn the input - initial co-states/total time map. Relevant examples can be found in \cite{cheng2018real,tang2019data,zang2022machine} for spacecraft applications.
% In \cite{cheng2018real} a NN was used to learn the aforementioned map for an orbit spacecraft transfer problem. A similar approach can be found in \cite{zang2022machine} for the landing problem. Instead, the kNN algorithm was use for learning the same map in \cite{tang2019data}. 
Anyway, these examples still have to solve the TPBVP.
% ------------------ state feedback ------------------ %
State feedback methods are based on the fact that the OCP solution is a function of the state. In \cite{sanchez2018real,zhu2019deep}, the state-feedback map was learned for the optimal landing problem using a Neural Network (NN), while quadcopter applications can be found in \cite{tailor2019learning, ferede2024end}. Note that, these examples do not guarantee satisfaction of Boundary Conditions (BCs) in hard sense.
% ------------------ parameterized solutions ------------------ %
Other approaches focus on producing a complete sequence of the trajectory and/or controls. 
In \cite{tang2018learning, banerjee2020learning} the whole sequence of the solution is learned and used to warm-up an optimizer.
% In \cite{tang2018learning} the complete sequence of states, controls and total time is learned from off-line OCP solutions. In the deployment phase, the predicted trajectories are then refined by means of a QP.
% Similarly, in \cite{banerjee2020learning} the solution trajectory for a spacecraft application is parameterized by $19$ cubic splines; also in this case, the learned map is used to warm up a sequential convex programming.  Multi-phase problems were addressed in \cite{wu2024deep}, where switching times were predicted by means of a NN.
An autoencoder-based approach is used in
\cite{berniker2015deep} for learning arm movements.
% First an autoencoder is trained to find a (latent) reduced representation of the trajectories and second a map from the inputs to the latent representation is trained. 
However, these approaches suffer from the fact that either the length or the resolution of the output are fixed.
% ----------------- recurrent neural networks ----------------- %
Recurrent NNs examples applied to TO can be found in \cite{Bency2019} for the Long-Short-Term-Memory \cite{hochreiter1997long} architecture while Transformer Model \cite{vaswani2017attention} was employed in \cite{guffanti2024transformers, celestini2024transformer, briden2023constraint}.
% , optimal solutions were learned throught a GPT architecture.
% that predicts future states and controls based on actual states/controls and cost-to-go. 
However, these examples do not guarantee BC satisfaction.

% However, these methods do not leverage prior information on the solution and do not guarantee BCs satisfaction. % in the hard sense.
% ----------------- The Enemy ----------------- %
% \subsection{Contributions}

In light of the above, learning solutions from data is promising for RT applications but 
% solving OCPs in the context of TO, particularly for minimum-energy problems, is computationally expensive. Therefore, it is difficult to meet RT requirements. As shown in the literature, data-driven methods offer a promising solution. However, 
existing methods: (i) do not impose BCs as hard constraints, (ii) do not leverage prior knowledge, (iii) still need numerical routines, or, (iv) have a predetermined length/resolution for the output. 

% ----------------- The Hero ----------------- %
In this paper, we overcome the aforementioned issues, starting from the following idea.
The planning problem of a generic Point-To-Point (PTP) motion in a fixed time is a solved problem \cite{biagiotti2008trajectory}. The only missing part is the quantity that steers a standard (or \textit{prior}) trajectory toward an optimal one. Focusing on this part enables (i) the design of a regressor that embeds BCs as hard constraints, and (ii) reduce the required data.
% ----------------- The Sword ----------------- %
This approach mimics the idea of \textit{residual learning} \cite{he2016deep}.
% , where only the informative part is learned. 
Resuming, the contribution is the \textbf{real-time} generation of near-minimum-energy trajectories for fixed end-point, fixed-time planning problems. This is reached using a \textbf{residual learning} paradigm, where only the informative part of the OCP solution is learned, allowing the embedding BCs as \textbf{hard constraints} and allowing deciding the resolution of the solution.
The proposed method is tested using two variational regression frameworks, namely NN ensembles and Gaussian Processes. Active learning (AL) capabilities are evaluated for both the regressors.
% The proposed method is validated through simulation experiments on three mechanical systems: a pendulum, a SCARA robot, and a six-axis manipulator.

Simulated experiments on three robotic systems (a pendulum, a SCARA, and a six-axis manipulator) are used to validate the method.

% \cite{tordesillas2023deep}
% The paper is organized as follows: Section~\ref{sec:method} outlines the methodology, Section~\ref{sec:result} presents the numerical experiments, and Section~\ref{sec:conclu} provides the conclusions.

